Disentangling the Cosmic Web Towards FRB 190608

FRB 190608 was detected by ASKAP and localized to a spiral galaxy at $z_{host}=0.11778$ in the SDSS footprint. The burst has a large dispersion measure ($DM_{FRB}=339.8$ $pc/cm^3$) compared to the expected cosmic average at its redshift. It also has a large rotation measure ($RM_{FRB}=353$ $rad/m^2$) and scattering timescale ($\tau=3.3$ $ms$ at $1.28$ $GHz$). Chittidi et al (2020) perform a detailed analysis of the ultraviolet and optical emission of the host galaxy and estimate the host DM contribution to be $110\pm 37$ $pc/cm^3$. This work complements theirs and reports the analysis of the optical data of galaxies in the foreground of FRB 190608 to explore their contributions to the FRB signal. Together, the two manuscripts delineate an observationally driven, end-to-end study of matter distribution along an FRB sightline; the first study of its kind. Combining KCWI observations and public SDSS data, we estimate the expected cosmic dispersion measure $DM_{cosmic}$ along the sightline to FRB 190608. We first estimate the contribution of hot, ionized gas in intervening virialized halos ($DM_{halos} \approx 7-28$ $pc/cm^3$). Then, using the Monte Carlo Physarum Machine (MCPM) methodology, we produce a 3D map of ionized gas in cosmic web filaments and compute the DM contribution from matter outside halos ($DM_{IGM} \approx 91-126$ $pc/cm^3$). This implies a greater fraction of ionized gas along this sightline is extant outside virialized halos. We also investigate whether the intervening halos can account for the large FRB rotation measure and pulse width and conclude that it is implausible. Both the pulse broadening and the large Faraday rotation likely arise from the progenitor environment or the host galaxy.

==> object_tab_full.tex <==
\begin{table*}
\centering
\caption{\footnotesize Properties of the foreground spectroscopic galaxies from SDSS$(\rho)$\label{tab:fg_gals}}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
RA & Dec & u & g & r & i & z & Redshift & $b$ & $\log(M_*/M_\odot)$ & $\log(M_{halo}/M_\odot)$ \\
$\deg$ & $\deg$ & mag & mag & mag & mag & mag &  & kpc &  &  \\
\hline
334.00914 & -7.87554 & 18.73 & 17.54 & 16.98 & 16.63 & 16.37 & 0.09122 & 158 & 10.36 & 11.81 \\
333.97368 & -7.87678 & 19.28 & 17.87 & 16.95 & 16.50 & 16.20 & 0.08544 & 300 & 10.59 & 12.09 \\
333.88476 & -8.01812 & 18.48 & 17.39 & 16.92 & 16.72 & 16.59 & 0.02732 & 367 & 9.06 & 11.04 \\
334.01930 & -8.02294 & 18.31 & 16.58 & 15.74 & 15.38 & 15.13 & 0.06038 & 541 & 10.63 & 12.17 \\
334.04856 & -7.79251 & 19.89 & 17.99 & 17.05 & 16.63 & 16.19 & 0.07745 & 597 & 10.54 & 12.01 \\
333.77207 & -7.53690 & 19.79 & 17.99 & 17.51 & 17.24 & 17.01 & 0.02394 & 784 & 8.85 & 10.95 \\
334.07667 & -7.76554 & 19.43 & 18.24 & 17.39 & 16.96 & 16.61 & 0.08110 & 819 & 10.37 & 11.82 \\
333.99058 & -8.10044 & 19.97 & 18.48 & 17.88 & 17.47 & 17.30 & 0.06522 & 951 & 9.75 & 11.39 \\
334.08866 & -8.01256 & 18.95 & 18.38 & 17.29 & 16.84 & 16.56 & 0.11726 & 1050 & 10.91 & 12.79 \\
334.12864 & -8.08630 & 19.20 & 17.86 & 17.31 & 16.96 & 16.75 & 0.07096 & 1091 & 10.01 & 11.55 \\
334.02532 & -8.14275 & 18.78 & 17.10 & 16.26 & 15.88 & 15.65 & 0.06755 & 1177 & 10.52 & 11.99 \\
334.05952 & -8.10454 & 19.59 & 17.68 & 16.75 & 16.35 & 16.05 & 0.08344 & 1225 & 10.62 & 12.14 \\
334.06830 & -8.16352 & 19.24 & 17.94 & 17.25 & 16.81 & 16.51 & 0.06718 & 1290 & 10.15 & 11.64 \\
334.10575 & -7.68905 & 17.71 & 18.08 & 17.60 & 17.31 & 17.63 & 0.08188 & 1295 & 9.63 & 11.34 \\
333.78314 & -7.91971 & 18.06 & 16.87 & 16.00 & 15.56 & 15.23 & 0.08274 & 1362 & 10.96 & 12.92 \\
334.22574 & -8.06238 & 19.63 & 17.91 & 17.00 & 16.66 & 16.27 & 0.07515 & 1389 & 10.41 & 11.85 \\
336.92314 & -9.72690 & 21.18 & 19.75 & 19.37 & 19.18 & 19.34 & 0.00548 & 1431 & 6.61 & 9.98 \\
336.87332 & -9.66743 & 22.38 & 21.00 & 20.22 & 19.98 & 20.05 & 0.00561 & 1434 & 6.64 & 9.99 \\
334.15962 & -7.75304 & 19.02 & 18.18 & 17.46 & 24.36 & 21.22 & 0.10573 & 1445 & 8.68 & 10.91 \\
336.87792 & -9.66500 & 16.64 & 15.65 & 15.35 & 15.33 & 15.24 & 0.00566 & 1447 & 8.08 & 10.60 \\
332.58598 & -9.19206 & 17.35 & 16.45 & 16.10 & 15.96 & 15.80 & 0.01059 & 1550 & 8.42 & 10.75 \\
334.20682 & -7.67446 & 18.38 & 16.96 & 16.43 & 16.09 & 15.84 & 0.07655 & 1567 & 10.44 & 11.89 \\
335.25023 & -9.64171 & 18.22 & 17.55 & 17.26 & 17.11 & 16.83 & 0.00968 & 1570 & 7.85 & 10.51 \\
333.30585 & -7.55163 & 17.48 & 15.82 & 14.99 & 14.57 & 14.35 & 0.02684 & 1581 & 10.26 & 11.70 \\
334.19822 & -8.17301 & 18.70 & 17.22 & 16.36 & 15.90 & 15.57 & 0.06969 & 1617 & 10.65 & 12.19 \\
334.23512 & -8.15220 & 18.79 & 17.34 & 16.37 & 15.94 & 15.56 & 0.07140 & 1678 & 10.73 & 12.35 \\
333.63069 & -7.83000 & 18.28 & 17.02 & 16.30 & 16.02 & 15.83 & 0.06014 & 1691 & 10.30 & 11.75 \\
333.95340 & -8.17987 & 21.32 & 18.43 & 17.51 & 17.06 & 16.73 & 0.08429 & 1702 & 10.52 & 11.99 \\
334.18224 & -8.14188 & 20.25 & 18.50 & 17.81 & 17.43 & 17.22 & 0.08413 & 1716 & 10.00 & 11.54 \\
333.97869 & -7.60364 & 21.10 & 18.63 & 17.75 & 17.35 & 17.13 & 0.08586 & 1780 & 10.24 & 11.71 \\
334.29543 & -8.03003 & 18.14 & 16.30 & 15.61 & 15.24 & 14.95 & 0.08515 & 1801 & 10.92 & 12.83 \\
334.21641 & -8.20391 & 18.95 & 17.31 & 16.44 & 16.01 & 15.73 & 0.07075 & 1819 & 10.57 & 12.07 \\
333.60751 & -8.39202 & 18.37 & 17.33 & 16.98 & 16.78 & 16.57 & 0.03864 & 1824 & 9.29 & 11.15 \\
334.26723 & -8.10378 & 19.60 & 17.70 & 16.67 & 16.17 & 15.86 & 0.08480 & 1893 & 10.81 & 12.53 \\
334.01393 & -8.21901 & 19.10 & 17.58 & 16.69 & 16.27 & 16.03 & 0.08488 & 1900 & 10.62 & 12.14 \\
334.30759 & -8.16872 & 19.93 & 17.85 & 17.16 & 16.80 & 16.56 & 0.07106 & 1980 & 10.14 & 11.63 \\
334.38681 & -8.03306 & 19.18 & 18.08 & 17.52 & 17.47 & 17.10 & 0.07334 & 2011 & 9.70 & 11.37 \\
333.72747 & -8.08445 & 20.61 & 18.58 & 17.71 & 17.30 & 17.04 & 0.08517 & 2045 & 10.21 & 11.69 \\
334.28010 & -8.29432 & 19.03 & 17.20 & 16.29 & 15.88 & 15.60 & 0.06086 & 2064 & 10.52 & 11.98 \\
334.26433 & -8.24452 & 19.76 & 18.17 & 17.39 & 16.94 & 16.55 & 0.07021 & 2106 & 10.23 & 11.69 \\
333.96086 & -7.55109 & 19.28 & 18.33 & 17.71 & 17.37 & 17.21 & 0.08645 & 2119 & 9.92 & 11.50 \\
334.47773 & -8.52306 & 17.26 & 15.69 & 14.90 & 14.50 & 14.31 & 0.03757 & 2140 & 10.54 & 12.01 \\
334.24456 & -8.28273 & 19.31 & 18.33 & 17.78 & 17.44 & 17.21 & 0.06988 & 2205 & 9.74 & 11.39 \\
334.19387 & -7.55411 & 18.21 & 17.15 & 16.39 & 15.97 & 15.58 & 0.08190 & 2207 & 10.76 & 12.42 \\
333.31567 & -7.32113 & 26.54 & 22.07 & 20.87 & 20.21 & 20.25 & 0.03359 & 2255 & 9.07 & 11.05 \\
334.09534 & -8.20804 & 19.95 & 18.45 & 17.48 & 16.95 & 16.53 & 0.10454 & 2273 & 10.71 & 12.32 \\
333.90661 & -8.26341 & 18.99 & 17.30 & 16.32 & 15.88 & 15.55 & 0.08559 & 2279 & 10.87 & 12.70 \\
334.29215 & -7.56561 & 19.03 & 17.23 & 16.38 & 15.99 & 15.75 & 0.07667 & 2314 & 10.60 & 12.11 \\
334.30767 & -7.57648 & 18.27 & 17.49 & 16.97 & 16.61 & 16.55 & 0.07721 & 2337 & 9.97 & 11.53 \\
334.08314 & -7.34866 & 19.31 & 18.44 & 18.28 & 17.91 & 18.19 & 0.05912 & 2352 & 8.92 & 10.99 \\
333.33125 & -9.59619 & 19.62 & 18.41 & 17.97 & 17.80 & 17.61 & 0.01704 & 2358 & 8.25 & 10.68 \\
334.58299 & -7.87911 & 19.73 & 18.29 & 17.85 & 17.50 & 17.30 & 0.05882 & 2362 & 9.58 & 11.30 \\
334.09968 & -8.29849 & 20.08 & 18.19 & 17.23 & 16.82 & 16.49 & 0.08407 & 2396 & 10.47 & 11.93 \\
334.16145 & -8.24709 & 19.34 & 18.09 & 17.44 & 17.05 & 17.11 & 0.09252 & 2406 & 10.11 & 11.62 \\
334.45061 & -7.52442 & 18.66 & 17.89 & 17.41 & 17.20 & 17.03 & 0.05942 & 2424 & 9.50 & 11.27 \\
334.05092 & -8.31494 & 20.07 & 17.59 & 16.58 & 16.02 & 15.60 & 0.08542 & 2489 & 11.02 & 13.09 \\
335.08261 & -8.77141 & 17.51 & 16.67 & 16.30 & 16.11 & 15.96 & 0.02431 & 2492 & 9.09 & 11.05 \\
334.85867 & -7.49905 & 19.95 & 17.97 & 17.68 & 17.40 & 17.52 & 0.03724 & 2535 & 8.98 & 11.01 \\
334.55416 & -7.93014 & 18.77 & 17.64 & 17.04 & 16.77 & 16.64 & 0.06804 & 2568 & 9.95 & 11.51 \\
333.92636 & -8.32121 & 17.80 & 16.21 & 15.43 & 15.02 & 14.73 & 0.08566 & 2586 & 11.08 & 13.25 \\
333.59107 & -8.04178 & 19.14 & 18.05 & 17.51 & 17.11 & 16.93 & 0.08287 & 2598 & 10.02 & 11.56 \\
333.92862 & -8.33754 & 18.35 & 17.03 & 16.24 & 15.84 & 15.54 & 0.08282 & 2598 & 10.76 & 12.43 \\
334.54320 & -7.85338 & 19.95 & 17.59 & 16.68 & 16.28 & 15.92 & 0.07058 & 2607 & 10.62 & 12.13 \\
334.39963 & -7.68859 & 19.91 & 18.47 & 17.57 & 17.10 & 16.67 & 0.08716 & 2613 & 10.44 & 11.90 \\
333.61659 & -8.08615 & 19.75 & 17.73 & 16.73 & 16.28 & 15.98 & 0.08523 & 2623 & 10.73 & 12.36 \\
333.87097 & -8.32608 & 21.20 & 18.69 & 17.71 & 17.19 & 17.08 & 0.08331 & 2635 & 10.29 & 11.75 \\
333.83482 & -8.32060 & 20.74 & 18.73 & 17.78 & 17.29 & 16.96 & 0.08295 & 2671 & 10.32 & 11.77 \\
334.98215 & -7.69106 & 18.40 & 16.56 & 15.67 & 15.27 & 14.95 & 0.03728 & 2685 & 10.35 & 11.79 \\
335.24209 & -9.39807 & 18.67 & 17.88 & 17.57 & 17.49 & 17.27 & 0.01852 & 2694 & 8.24 & 10.68 \\
334.96020 & -7.53119 & 19.35 & 18.25 & 17.83 & 17.65 & 17.64 & 0.03721 & 2752 & 8.89 & 10.97 \\
333.51245 & -8.23405 & 18.79 & 17.73 & 17.16 & 16.83 & 16.54 & 0.06459 & 2789 & 9.96 & 11.51 \\
334.52427 & -7.69061 & 18.81 & 18.05 & 17.21 & 16.84 & 16.55 & 0.07366 & 2819 & 10.27 & 11.73 \\
334.57786 & -7.53228 & 18.91 & 17.95 & 17.46 & 17.13 & 17.04 & 0.05943 & 2834 & 9.59 & 11.31 \\
334.48028 & -8.03480 & 18.85 & 18.24 & 17.76 & 17.38 & 17.38 & 0.08621 & 2860 & 9.73 & 11.39 \\
333.63124 & -8.19488 & 20.80 & 18.81 & 17.89 & 17.43 & 17.09 & 0.08471 & 2872 & 10.26 & 11.73 \\
333.62787 & -7.55990 & 17.64 & 16.43 & 15.73 & 15.31 & 15.04 & 0.07974 & 2883 & 10.89 & 12.74 \\
335.05644 & -7.64594 & 18.29 & 16.83 & 15.95 & 15.56 & 15.22 & 0.03709 & 2897 & 10.22 & 11.67 \\
333.92849 & -7.43108 & 20.21 & 18.48 & 17.65 & 17.24 & 16.88 & 0.08778 & 2904 & 10.28 & 11.75 \\
334.60195 & -8.01414 & 17.82 & 16.82 & 16.26 & 15.93 & 15.76 & 0.07045 & 2940 & 10.30 & 11.76 \\
334.35248 & -7.46392 & 19.54 & 17.51 & 16.65 & 16.21 & 15.93 & 0.07682 & 2951 & 10.59 & 12.10 \\
335.27252 & -7.66024 & 19.06 & 18.26 & 17.74 & 17.69 & 17.50 & 0.03147 & 2956 & 8.73 & 10.89 \\
334.17675 & -8.42280 & 20.22 & 18.25 & 17.52 & 17.10 & 16.72 & 0.07777 & 2994 & 10.23 & 11.70 \\
333.63525 & -7.87152 & 19.68 & 17.83 & 16.82 & 16.46 & 16.17 & 0.11691 & 3002 & 10.85 & 12.64 \\
333.52742 & -8.07692 & 19.09 & 17.32 & 16.37 & 15.95 & 15.65 & 0.08365 & 3035 & 10.80 & 12.51 \\
335.10460 & -7.63059 & 18.38 & 17.11 & 16.45 & 16.34 & 16.17 & 0.03739 & 3057 & 9.64 & 11.32 \\
333.65414 & -8.04665 & 19.13 & 18.52 & 17.51 & 17.08 & 16.80 & 0.11687 & 3076 & 10.73 & 12.36 \\
333.87948 & -8.40637 & 21.57 & 18.72 & 17.66 & 17.56 & 17.04 & 0.08372 & 3082 & 10.37 & 11.82 \\
334.85468 & -8.66114 & 19.40 & 17.78 & 17.12 & 16.64 & 16.27 & 0.03712 & 3082 & 9.73 & 11.37 \\
333.84272 & -8.38191 & 19.37 & 18.07 & 17.43 & 17.06 & 16.71 & 0.08603 & 3084 & 10.24 & 11.71 \\
334.18338 & -8.40637 & 19.62 & 17.29 & 16.33 & 15.92 & 15.55 & 0.08428 & 3139 & 10.94 & 12.87 \\
333.94420 & -8.37594 & 18.61 & 17.28 & 16.63 & 16.25 & 15.90 & 0.09405 & 3140 & 10.66 & 12.22 \\
334.52319 & -8.42892 & 18.18 & 16.64 & 15.78 & 15.32 & 14.86 & 0.06006 & 3141 & 10.82 & 12.56 \\
334.01727 & -8.42051 & 19.85 & 18.52 & 17.63 & 17.19 & 16.98 & 0.08640 & 3143 & 10.26 & 11.73 \\
333.59592 & -8.31188 & 18.30 & 17.21 & 16.43 & 15.99 & 15.69 & 0.07673 & 3185 & 10.65 & 12.20 \\
331.57082 & -8.55208 & 16.65 & 15.66 & 15.11 & 14.83 & 14.49 & 0.01697 & 3223 & 9.56 & 11.27 \\
334.46675 & -8.29629 & 18.60 & 16.94 & 16.03 & 15.64 & 15.43 & 0.07704 & 3229 & 10.75 & 12.40 \\
333.98541 & -8.35492 & 18.78 & 17.46 & 16.74 & 16.45 & 16.29 & 0.10382 & 3246 & 10.58 & 12.07 \\
334.59352 & -7.58519 & 18.69 & 18.16 & 17.66 & 17.39 & 17.17 & 0.07148 & 3288 & 9.68 & 11.36 \\
334.57936 & -7.56042 & 19.96 & 18.58 & 17.69 & 17.34 & 17.02 & 0.07260 & 3337 & 10.07 & 11.59 \\
334.18679 & -8.54514 & 20.26 & 18.36 & 17.41 & 17.00 & 16.62 & 0.07064 & 3346 & 10.28 & 11.74 \\
333.23266 & -7.81058 & 18.12 & 16.61 & 15.70 & 15.26 & 14.96 & 0.06023 & 3394 & 10.78 & 12.46 \\
333.80390 & -8.41952 & 20.33 & 18.41 & 17.57 & 17.11 & 16.79 & 0.08682 & 3405 & 10.35 & 11.80 \\
337.77493 & -0.19552 & 17.90 & 17.10 & 16.89 & 16.77 & 16.55 & 0.00518 & 3406 & 7.38 & 10.30 \\
335.13939 & -8.46544 & 17.18 & 15.83 & 15.08 & 14.68 & 14.32 & 0.03723 & 3422 & 10.53 & 12.00 \\
333.44084 & -8.02410 & 18.98 & 17.80 & 17.19 & 16.83 & 16.70 & 0.08399 & 3444 & 10.17 & 11.66 \\
333.52486 & -8.21035 & 18.54 & 17.11 & 16.53 & 16.16 & 15.98 & 0.08504 & 3447 & 10.50 & 11.97 \\
334.39958 & -8.34509 & 19.61 & 17.45 & 16.55 & 16.11 & 15.79 & 0.08483 & 3457 & 10.79 & 12.48 \\
337.65333 & -0.11028 & 18.01 & 17.13 & 16.99 & 16.96 & 17.05 & 0.00527 & 3475 & 7.20 & 10.23 \\
333.69536 & -8.38416 & 19.16 & 18.10 & 17.40 & 16.96 & 16.64 & 0.08580 & 3483 & 10.31 & 11.77 \\
335.14405 & -8.49335 & 17.92 & 16.10 & 15.31 & 14.87 & 14.53 & 0.03746 & 3489 & 10.49 & 11.94 \\
332.74066 & -8.98288 & 21.73 & 20.02 & 19.24 & 18.99 & 19.34 & 0.02813 & 3499 & 8.33 & 10.72 \\
333.48582 & -8.20474 & 19.71 & 18.29 & 17.87 & 17.54 & 17.45 & 0.08296 & 3546 & 9.78 & 11.42 \\
334.68442 & -8.97613 & 16.72 & 15.76 & 15.36 & 15.08 & 14.85 & 0.03818 & 3555 & 10.01 & 11.53 \\
334.72528 & -7.75997 & 18.10 & 17.10 & 16.21 & 15.77 & 15.47 & 0.07089 & 3583 & 10.76 & 12.42 \\
334.72042 & -7.71679 & 19.44 & 18.49 & 18.07 & 17.77 & 17.57 & 0.07102 & 3614 & 9.47 & 11.25 \\
333.77296 & -7.34495 & 20.00 & 17.98 & 17.04 & 16.63 & 16.31 & 0.08623 & 3634 & 10.57 & 12.06 \\
334.72957 & -7.73642 & 18.92 & 17.34 & 16.49 & 15.97 & 15.59 & 0.07175 & 3669 & 10.69 & 12.27 \\
334.74632 & -7.77252 & 19.34 & 17.72 & 16.81 & 16.40 & 16.09 & 0.07093 & 3676 & 10.45 & 11.90 \\
334.59850 & -7.96627 & 19.03 & 17.96 & 17.37 & 17.06 & 16.80 & 0.09237 & 3688 & 10.15 & 11.65 \\
334.35803 & -8.42539 & 18.33 & 16.83 & 15.91 & 15.50 & 15.24 & 0.08468 & 3691 & 10.94 & 12.88 \\
339.82785 & -1.70077 & 22.45 & 22.21 & 21.69 & 21.79 & 21.82 & 0.00574 & 3730 & 5.91 & 9.69 \\
333.42181 & -8.15614 & 19.31 & 18.28 & 17.64 & 17.24 & 17.03 & 0.08268 & 3736 & 10.05 & 11.57 \\
333.58751 & -8.37585 & 19.75 & 17.61 & 16.70 & 16.27 & 15.97 & 0.08360 & 3746 & 10.70 & 12.30 \\
333.44813 & -8.21684 & 18.40 & 17.31 & 16.86 & 16.51 & 16.44 & 0.08285 & 3764 & 10.11 & 11.62 \\
333.37250 & -8.04408 & 20.18 & 18.12 & 17.15 & 16.71 & 16.37 & 0.08235 & 3789 & 10.55 & 12.03 \\
334.14376 & -8.53156 & 20.48 & 18.66 & 17.78 & 17.38 & 17.03 & 0.08431 & 3798 & 10.22 & 11.69 \\
339.34208 & -8.46260 & 22.17 & 20.43 & 18.67 & 18.98 & 20.57 & 0.00942 & 3813 & 7.46 & 10.34 \\
337.21986 & -8.45558 & 18.88 & 18.35 & 17.86 & 17.68 & 17.57 & 0.01591 & 3875 & 8.13 & 10.63 \\
334.61148 & -7.62855 & 19.83 & 18.59 & 17.74 & 17.30 & 17.02 & 0.08623 & 3877 & 10.24 & 11.71 \\
334.44610 & -8.33022 & 19.69 & 18.22 & 17.25 & 16.84 & 16.44 & 0.09300 & 3883 & 10.59 & 12.10 \\
333.81744 & -9.26324 & 17.11 & 15.28 & 14.57 & 14.19 & 13.94 & 0.03839 & 3904 & 10.66 & 12.23 \\
335.68486 & -7.68138 & 19.03 & 16.96 & 16.40 & 16.06 & 15.84 & 0.03202 & 3958 & 9.69 & 11.34 \\
333.84965 & -8.41284 & 19.83 & 18.36 & 17.64 & 17.30 & 17.09 & 0.10753 & 3958 & 10.30 & 11.77 \\
333.40420 & -7.98087 & 19.20 & 17.71 & 16.81 & 16.43 & 16.18 & 0.09526 & 4041 & 10.62 & 12.15 \\
335.33134 & -8.61088 & 19.80 & 18.46 & 17.63 & 17.42 & 17.05 & 0.03701 & 4046 & 9.38 & 11.19 \\
332.88068 & -9.45415 & 18.53 & 17.58 & 17.42 & 17.29 & 16.96 & 0.02825 & 4048 & 8.69 & 10.88 \\
333.03820 & -8.14585 & 19.85 & 18.13 & 17.27 & 16.88 & 16.59 & 0.05592 & 4049 & 10.00 & 11.53 \\
333.01463 & -7.57893 & 16.51 & 14.92 & 14.16 & 13.82 & 13.64 & 0.05370 & 4066 & 11.06 & 13.19 \\
337.69336 & 1.39594 & 21.15 & 21.05 & 20.67 & 20.85 & 21.22 & 0.00531 & 4069 & 6.00 & 9.72 \\
334.34135 & -8.52456 & 18.99 & 17.45 & 16.57 & 16.18 & 15.87 & 0.08386 & 4116 & 10.66 & 12.22 \\
333.31693 & -7.80027 & 19.45 & 17.88 & 17.27 & 16.89 & 16.64 & 0.08384 & 4118 & 10.22 & 11.70 \\
333.74036 & -8.60162 & 19.19 & 17.83 & 16.90 & 16.40 & 16.15 & 0.07831 & 4162 & 10.56 & 12.04 \\
339.95627 & -8.38966 & 22.82 & 21.60 & 21.05 & 21.31 & 21.28 & 0.00930 & 4188 & 6.41 & 9.90 \\
332.99740 & -8.12135 & 19.54 & 17.88 & 17.05 & 16.66 & 16.35 & 0.05601 & 4191 & 10.09 & 11.59 \\
335.36315 & -8.64717 & 17.11 & 15.54 & 14.63 & 14.22 & 13.82 & 0.03727 & 4198 & 10.81 & 12.54 \\
333.02767 & -7.85184 & 18.69 & 17.74 & 17.10 & 16.72 & 16.45 & 0.05970 & 4222 & 9.98 & 11.52 \\
332.97939 & -8.05705 & 19.13 & 18.10 & 17.70 & 17.47 & 17.24 & 0.05645 & 4246 & 9.38 & 11.20 \\
333.58269 & -8.47572 & 19.75 & 18.09 & 17.15 & 16.75 & 16.44 & 0.08431 & 4248 & 10.47 & 11.92 \\
333.69440 & -7.46208 & 19.70 & 18.29 & 17.58 & 17.25 & 17.08 & 0.11737 & 4279 & 10.38 & 11.84 \\
333.22076 & -8.92340 & 19.19 & 17.88 & 17.47 & 17.12 & 17.08 & 0.04521 & 4279 & 9.38 & 11.20 \\
333.66330 & -8.68562 & 18.66 & 17.22 & 16.55 & 16.16 & 15.87 & 0.07013 & 4296 & 10.41 & 11.86 \\
334.97959 & -9.11178 & 18.28 & 17.37 & 16.97 & 16.69 & 16.43 & 0.03788 & 4305 & 9.37 & 11.19 \\
333.79934 & -8.73099 & 17.32 & 16.07 & 15.40 & 14.99 & 14.71 & 0.07066 & 4316 & 10.90 & 12.78 \\
340.31075 & -0.61684 & 21.61 & 21.20 & 21.26 & 21.92 & 22.83 & 0.00586 & 4321 & 5.39 & 9.46 \\
335.58784 & -8.13058 & 17.05 & 15.85 & 15.16 & 14.79 & 14.61 & 0.03750 & 4345 & 10.38 & 11.82 \\
340.31016 & -0.61787 & 16.99 & 16.30 & 15.98 & 15.73 & 15.82 & 0.00590 & 4345 & 7.88 & 10.52 \\
334.14184 & -8.51142 & 18.36 & 17.35 & 16.85 & 16.53 & 16.26 & 0.10219 & 4368 & 10.38 & 11.84 \\
333.52740 & -7.41960 & 19.64 & 17.60 & 16.73 & 16.35 & 16.08 & 0.09257 & 4376 & 10.66 & 12.21 \\
334.83052 & -7.57037 & 20.32 & 17.94 & 16.94 & 16.61 & 16.10 & 0.07119 & 4380 & 10.58 & 12.07 \\
340.30886 & -0.62085 & 17.79 & 17.02 & 16.72 & 16.59 & 16.12 & 0.00595 & 4381 & 7.71 & 10.45 \\
333.77111 & -8.47030 & 18.68 & 17.34 & 16.64 & 16.28 & 16.02 & 0.10333 & 4396 & 10.71 & 12.31 \\
333.45157 & -7.82720 & 19.59 & 17.60 & 16.60 & 16.18 & 15.82 & 0.11672 & 4454 & 11.04 & 13.16 \\
333.53113 & -8.64312 & 19.60 & 18.68 & 18.19 & 17.86 & 17.67 & 0.07072 & 4456 & 9.48 & 11.26 \\
333.35324 & -9.28117 & 16.71 & 15.63 & 15.27 & 14.99 & 14.91 & 0.03974 & 4480 & 10.02 & 11.54 \\
336.13738 & -9.21193 & 17.96 & 16.92 & 16.51 & 16.29 & 16.05 & 0.02423 & 4492 & 9.14 & 11.07 \\
335.05289 & -8.10998 & 19.05 & 17.53 & 16.70 & 16.27 & 15.88 & 0.05995 & 4500 & 10.38 & 11.82 \\
333.28084 & -8.43766 & 19.30 & 18.16 & 17.51 & 17.11 & 16.84 & 0.06984 & 4508 & 10.01 & 11.54 \\
334.72167 & -8.47573 & 19.80 & 18.19 & 17.77 & 17.59 & 17.59 & 0.07060 & 4526 & 9.53 & 11.28 \\
330.84321 & -9.29951 & 17.56 & 16.20 & 15.81 & 15.55 & 15.54 & 0.01746 & 4539 & 9.14 & 11.07 \\
333.74317 & -8.47739 & 19.73 & 18.37 & 17.77 & 17.35 & 16.94 & 0.10389 & 4543 & 10.33 & 11.79 \\
337.59090 & -9.42039 & 18.95 & 17.67 & 17.15 & 16.93 & 16.96 & 0.01560 & 4544 & 8.50 & 10.79 \\
333.54397 & -8.52227 & 18.24 & 16.95 & 16.16 & 15.77 & 15.39 & 0.08371 & 4573 & 10.83 & 12.60 \\
333.34939 & -8.28668 & 18.83 & 18.61 & 17.75 & 17.36 & 16.87 & 0.08574 & 4596 & 10.62 & 12.14 \\
333.15297 & -7.51910 & 20.22 & 19.47 & 19.25 & 18.82 & 18.83 & 0.06893 & 4601 & 8.81 & 10.95 \\
333.63780 & -8.41733 & 19.54 & 18.22 & 17.60 & 17.27 & 17.03 & 0.10540 & 4612 & 10.26 & 11.74 \\
333.42429 & -7.90740 & 19.98 & 17.83 & 16.86 & 16.52 & 16.23 & 0.11622 & 4614 & 10.82 & 12.57 \\
333.55117 & -8.52716 & 17.95 & 16.17 & 15.30 & 14.84 & 14.64 & 0.08466 & 4618 & 11.17 & 13.49 \\
335.48843 & -8.75065 & 18.93 & 17.28 & 16.40 & 16.02 & 15.64 & 0.03714 & 4620 & 10.05 & 11.55 \\
340.38117 & 0.39551 & 22.03 & 21.89 & 21.71 & 22.35 & 22.45 & 0.00582 & 4657 & 5.34 & 9.45 \\
333.60165 & -8.72915 & 18.95 & 17.87 & 17.37 & 17.21 & 16.99 & 0.07118 & 4685 & 9.72 & 11.38 \\
340.39115 & 0.40075 & 17.23 & 15.13 & 14.52 & 14.34 & 19.56 & 0.00588 & 4711 & 6.51 & 9.94 \\
333.46583 & -8.67298 & 18.73 & 16.91 & 16.04 & 15.61 & 15.28 & 0.07034 & 4738 & 10.77 & 12.44 \\
334.79673 & -8.20196 & 19.68 & 18.45 & 18.06 & 17.75 & 17.77 & 0.08186 & 4741 & 9.56 & 11.31 \\
331.75007 & -7.30866 & 17.95 & 16.84 & 16.37 & 16.10 & 15.87 & 0.02731 & 4745 & 9.40 & 11.19 \\
340.39093 & 0.40188 & 21.81 & 21.95 & 21.48 & 22.00 & 22.83 & 0.00593 & 4751 & 6.47 & 9.92 \\
337.31163 & 1.09886 & 21.71 & 20.09 & 19.10 & 18.73 & 18.51 & 0.00652 & 4786 & 7.42 & 10.32 \\
333.52278 & -8.72699 & 19.75 & 17.62 & 16.67 & 16.28 & 15.93 & 0.07012 & 4797 & 10.58 & 12.07 \\
334.84773 & -7.87095 & 19.59 & 18.26 & 17.80 & 17.52 & 17.25 & 0.08383 & 4806 & 9.87 & 11.47 \\
335.24304 & -7.60934 & 17.83 & 16.95 & 16.48 & 16.20 & 16.06 & 0.05335 & 4814 & 9.84 & 11.44 \\
333.73847 & -8.52122 & 20.26 & 18.27 & 17.22 & 16.81 & 16.47 & 0.10328 & 4814 & 10.72 & 12.32 \\
333.58549 & -8.58951 & 19.10 & 17.99 & 17.09 & 16.67 & 16.24 & 0.08531 & 4843 & 10.59 & 12.10 \\
333.49686 & -8.55770 & 19.69 & 17.64 & 16.65 & 16.24 & 15.93 & 0.08270 & 4850 & 10.72 & 12.34 \\
336.75393 & -8.31307 & 16.99 & 15.98 & 15.41 & 15.13 & 14.97 & 0.02369 & 4868 & 9.69 & 11.34 \\
334.47639 & -8.59211 & 20.21 & 18.72 & 17.79 & 17.38 & 17.03 & 0.08495 & 4908 & 10.25 & 11.72 \\
331.86877 & -8.85214 & 18.96 & 18.05 & 17.72 & 17.62 & 17.61 & 0.02827 & 4919 & 8.56 & 10.82 \\
333.20583 & -8.14084 & 20.68 & 18.48 & 17.41 & 16.83 & 16.67 & 0.08379 & 4927 & 10.52 & 12.00 \\
335.83552 & -7.80371 & 17.76 & 17.35 & 16.73 & 16.38 & 16.15 & 0.03712 & 4937 & 9.73 & 11.37 \\
335.82546 & -7.85494 & 18.30 & 16.73 & 15.86 & 15.44 & 15.09 & 0.03744 & 4945 & 10.28 & 11.73 \\
332.81881 & -8.13418 & 18.91 & 17.67 & 17.19 & 16.87 & 16.67 & 0.05654 & 4945 & 9.76 & 11.39 \\
331.59113 & -8.08997 & 16.02 & 14.39 & 13.69 & 13.34 & 13.11 & 0.02748 & 4953 & 10.67 & 12.24 \\
331.64024 & -8.03520 & 17.01 & 15.71 & 15.03 & 14.62 & 14.31 & 0.02821 & 4970 & 10.27 & 11.71 \\
334.87144 & -7.86497 & 19.07 & 17.25 & 16.32 & 15.84 & 15.42 & 0.08444 & 4977 & 10.93 & 12.86 \\
332.84547 & -8.27582 & 18.01 & 16.57 & 15.81 & 15.34 & 15.05 & 0.05650 & 4983 & 10.63 & 12.16 \\
\hline
\end{tabular}
\end{table*}

